On the Stability of Nonlinear Receding Horizon Control: A Geometric Perspective

%!TEX root = LCSS_main_max.tex The widespread adoption of nonlinear Receding Horizon Control (RHC) strategies by industry has led to more than 30 years of intense research efforts to provide stability guarantees for these methods. However, current theoretical guarantees require that each (generally nonconvex) planning problem can be solved to (approximate) global optimality, which is an unrealistic requirement for the derivative-based local optimization methods generally used in practical implementations of RHC. This paper takes the first step towards understanding stability guarantees for nonlinear RHC when the inner planning problem is solved to first-order stationary points, but not necessarily global optima. Special attention is given to feedback linearizable systems, and a mixture of positive and negative results are provided. We establish that, under certain strong conditions, first-order solutions to RHC exponentially stabilize linearizable systems. Surprisingly, these conditions can hold even in situations where there may be \textit{spurious local minima.} Crucially, this guarantee requires that state costs applied to the planning problems are in a certain sense `compatible' with the global geometry of the system, and a simple counter-example demonstrates the necessity of this condition. These results highlight the need to rethink the role of global geometry in the context of optimization-based control.

==> feedblack_lin.tex <==

%!TEX root = LCSS_main_max.tex

Feedback Linearizable systems are perhaps the most widely studied and well-characterized class of systems in the nonlinear geometric control literature. Roughly speaking, a system is feedback linearizable if it can be transformed into a linear system using state feedback and a coordinate transformation. Our introduction to this concept will be brief, since it is covered extensively by a number of standard references \cite{sastry2013nonlinear}. The usual method for checking if \eqref{eq:dynamics} is feedback linearizable is to first append and output $y \in \R^m$ to the system to obtain a new system of the form
\begin{align*}
    \dot{x} &= f(x) +g(x)u \\
    y &= h(x)
\end{align*}
where $y \in \R^m$ and $h \colon \R^n \to \R^m$  is a smooth map with the property that $h(0) =0$. The $j$-th output is the differentiated along the dynamics of the system until at least one inputs 'appears', resulting in an expression of the form
\begin{equation}
    y_j^{(\gamma_j)} = F_j(x) +\sum_{i=1}G_{ji}(x)u_i.
\end{equation}
where $u_i$ is the $i$-th  entry of the input, $\gamma_j$ is the number of times $y_j$ must be differentiated before an input appears in the expression for one of its time derivatives, and the $b_j$ and $a_{ji}$ are both  smooth functions. 
\begin{equation}
    \begin{bmatrix}
    y_1^{(\gamma_1)} & \dots &
    y_m^{(\gamma_m)}
    \end{bmatrix}^T = F(x) + G(x)u,
\end{equation}
where $F(x)$ is known as the \emph{drift term} and $G(x)$ is called the \emph{decoupling matrix}. In the case where $G(x)$ is bounded away from singularity for each $x \in \R^n$ the feedback law
\begin{equation}
    u(x,v) = G(x)^{-1}\left[-F(x) + v \right]
\end{equation}
produces the linear relationship
\begin{equation}
\begin{bmatrix}
    y_1^{(\gamma_1)} & \dots &
    y_m^{(\gamma_m)}
    \end{bmatrix}^T = \begin{bmatrix}
    v_1 & \dots &
    v_m
    \end{bmatrix}
\end{equation}
between the output and the new virtual input $v \in \R^m$. In the case that $\gamma_1 + \dots +\gamma_m =n$ then the outputs and their derivatives define a valid set of new coordinates $\xi = (\xi_1^1, \dots, \xi_1^{\gamma_1}, \dots, \xi_{m}^{1}, \dots,  \xi_m^{\gamma_m}) = (y_1, \dots, y_1^{(\gamma_1 -1)}, \dots, y_m, \dots, y_m^{(\gamma_m)}) \in \R^n $ for the system.Indeed, it can be shown that $\xi = \Phi(x)$, where $\Phi \colon \R^n\to \R^n$ is a diffeomorphism defining the coordinate transformation with the property that $\Phi(0) =0$. In the new coordinates the dynamics of the system are of the form
\begin{align}\label{eq:normal_form}
    \dot{\xi}_1^1 = \xi_1^2 & \ \ \  \dot{\xi}_1^2 = \xi_1^{3} & \dots  & \ \ \ \dot{\xi}_1^{(\gamma_1-1)} =\dot{\xi}_1^{\gamma_1} \\ \nonumber
    \vdots & & & \vdots\\ \nonumber
    \dot{\xi}_m^1 = \xi_m^2 & \ \ \  \dot{\xi}_m^2 = \xi_m^{3} & \dots  & \ \ \ \dot{\xi}_m^{(\gamma_m-1)} =\dot{\xi}_m^{\gamma_m}\\ \nonumber
\end{align}
\begin{equation*}
    \begin{bmatrix} 
    \dot{\xi}_1^{\gamma_1} & \dots & \dot{\xi}_1^{\gamma_1}
    \end{bmatrix} = \hat{F}(\xi) +\hat{A}(\xi)u
\end{equation*}
where $\hat{F}= F \circ \Phi$ and $\hat{G} = A \circ \Phi$. That is, in the new coordinates the dynamics are represented by $m$ linear integrator chains, which can be decoupled and controlled independently. These dynamic equations can be re-arranged into a compact representation of the form
\begin{equation}
    \dot{\xi} = \hat{A}\xi + \hat{B}[\hat{F}(\xi) + \hat{G}(\xi)u]
\end{equation}
where $A\in \R^{n\times n}$ and $B \in \R^{n \times m}$ are such that $(A,B)$ is a completely controllable pair. Applying the control law $u(\xi,v)$ yields
\begin{equation}
    \dot{\xi} = A\xi +Bv
\end{equation}



==> main_results.tex <==
%!TEX root = LCSS_main_max.tex


Using the novel model introduced above, we are now ready to investigate the stability properties of practical RHC control implementations. In an effort to provide stability guarantees which are agnostic to the particular choice of optimization algorithm, we focus our analysis on properties shared by all of the stationary points of the finite-horizon prediction problems. In Section \ref{subsec:exp_stable} we first provide a general results which demonstrates that if each stationary point of the finite horizon problems corresponds to an exponentially decaying system trajectory then $\PRHC$ can be guaranteed to be stabilizing by making $T>0$ sufficient large when compared to $\delta>0$. In Section \ref{subsec:fbl}, we provide sufficient conditions for the exponential decay condition to hold when the system is feedback linearizable. Finally, in Section \ref{subsec:examples} we examine several examples which demonstrate that $\PRHC$ can get stuck at undesirable equilibrium for all choices of $T\geq \delta >0$ if the stationary conditions for the finite horizon problems do not capture certain global structural properties of the system.  

\subsection{Exponentially Stable Stationary Points}\label{subsec:exp_stable}


\msnote{practical?}


\begin{lemma}\label{lemma:exp_converge}
Let Assumptions \ref{ass:growth}- \ref{ass:terminal} hold. Further assume that there exists positive constants $M, \alpha, K>0$ such that for each $x_0 \in \R^n$ and $T>0$ each stationary pair $(x^*(\cdot),u^*(\cdot))$ of $J_T(x_0,\cdot)$ satisfies the following conditions:
\begin{align}\label{eq:exp_bound}
    \| x^*(t)\|_2 &\leq M e^{-\alpha t} \| x_0\|\\ \nonumber
    \| u^*(\cdot)\|_2^2 &\leq K \| x_0\|_2
\end{align}
Then for each $\delta>0$ there exists $T(\delta)>0$ such that if $T> T(\delta)$ then $\text{RHC}(T,\delta)$ is exponentially stabilizing. 
\end{lemma}

\subsection{Feedback Linearizable Systems}\label{sec:fbl}
In this section, we will assume that the system \eqref{eq:dynamics} is full-state linearizable so that it can be put into the canonical form \eqref{eq:normal_form} via the coordinate change $\xi = \Phi(x)$ in which its dynamics are of the form
\begin{equation}
    \dot{\xi}=\hat{A}\xi + \hat{B}[\hat{F}(\xi) + \hat{G}(\xi)u)]
\end{equation}
Our convergence result will require that the representation of the dynamics in the $\xi$ coordinates satisfies the following regularity conditions:
\begin{assumption}\label{ass:fbl1}
There exists $\hat{L}>0$ and a constant matrix $\bar{G} \in \R^{n \times m}$ such that for each $\xi \in \R^n$
\begin{align*}
    \|\frac{d}{d\xi}\hat{F}(\xi)\|_2 &\leq \hat{L} \|\xi\|_2\\
    \hat{G}(\xi) &= \hat{G}
\end{align*}
\end{assumption}
We will also assume that the state and running cost satisfy the following geometric conditions:
\begin{assumption}\label{ass:fbl2}
The input running cost $R$ is strongly convex. Furthermore, the running cost $\hat{Q}$ and terminal cost $\hat{V}$ are both convex in the linearizing coordinates and there exists $\alpha_{\hat{Q}},\beta_{\hat{Q}}, \alpha_{\hat{V}} >0$ such that for each $\xi \in \R^n$ we have
\begin{align*}
     \beta_{\hat{Q}} \| \xi\|_2^2\leq \hat{Q}(\xi) &\leq \alpha_{\hat{Q}} \|\xi \|_2^2  \\
      0\leq \hat{V}(\xi)&\leq \alpha_{\hat{V}} \| \xi\|_2^2.
\end{align*}
\end{assumption}




\begin{lemma}\label{lemma:fbl}
Assume that \eqref{eq:dynamics} is feedback linearizable and that Assumptions \ref{ass:fbl1} and \ref{ass:fbl2} hold. Then if $\alpha_{R}\leq \frac{\beta_{\hat{G} }\sigma_{min}(\hat{G})^2}{16\hat{L}^2 }$ there exists $M,\alpha,K>0$ such that for each $t\geq 0$ and $x_0 \in \R^n$ each stationary pair $(x^*(\cdot),u^*(\cdot))$ of $J_T(x_0,\cdot)$ satisfies
\begin{align*}
\| x^*(t)\|_2 &\leq M e^{-\alpha t} \| x_0\|_2\\ \nonumber
    \| u^*(\cdot)\|_2^2 &\leq K \| x_0\|_2\end{align*}
\end{lemma}









\begin{theorem}\label{thm:fbl}
Assume that \eqref{eq:dynamics} is feedback linearizable and that the hyptheses of \ref{lemma:fbl} hold. Then for each $\delta >0$ there exists $T(\delta)>0$ such that if $T>T(\delta)$ then $\PRHC$ is exponentially stabilizing. 
\end{theorem}
\begin{proof}
The proof follows directly from Lemmas \ref{lemma:exp_converge} and \ref{lemma:fbl}
\end{proof}



\subsection{Examples}\label{sec:examples}

\subsubsection{Convergence for Inverted Pendulum}
\twnote{Will work through the dynamics of a double pendulum example and show that our stability result applies to this systems} 


\subsubsection{Relative Scaling of State and Input Costs}
Consider the scalar system 
\begin{equation}
    \dot{x} = \sin(x) + u
\end{equation}
\twnote{We will use this system to show that $\PRHC$ can, in fact, get stuck if the input cost is not scaled to be small enough compared o the state runing cost}

\subsubsection{Geometrically Incompatible State Costs}

Consider the system
\begin{equation}\label{eq:ex_bump}
   \begin{bmatrix}
   \dot{x}_1 \\
   \dot{x}_2
   \end{bmatrix} = \underbrace{\begin{bmatrix}
   -1 & 1 \\
   0 & 0
   \end{bmatrix}}_{A}\begin{bmatrix} 
   x_1 \\ x_2
   \end{bmatrix} + \underbrace{\begin{bmatrix} 
   0 \\ 1
   \end{bmatrix}}_Bu + \eta(x_1) \underbrace{\begin{bmatrix}
   10 \\0
   \end{bmatrix}}_{d}
\end{equation}
where $\eta \colon \R^n \to \R_{+}$ is any $C^\infty$ function which satisfies 
\begin{equation}
\eta_c(x_1) = 1  
\end{equation}
 Letting $x = (x_1, x_2)$, on the region $D_1 \colon = \set{(x_1,x_2) \colon x_1 \leq  \frac{1}{2}}$ the dynamics of \eqref{eq:ex_bump} are identical to the controllable linear system $\dot{x} = Ax + Bu$, while on the set $_22 = \set{(x_1,x_2) \colon x_1 \leq  \frac{1}{2}}$ the dynamics are affine and governed by $\dot{x} = Ax + Bu + d$. The reader may observe that \eqref{eq:ex_bump} is full-state input-output linearizable with the output $y =x_1$, and thus may be smoothly stabilized to the origin. Nonetheless,  we will show that natural choices for the running costs lead to undesirable equilibria for the practical receding horizon process in $D_2$.
 
 Unlike the previous example, the position of this equilibrium point is entirely determined by the interplay between the geometry of \eqref{eq:ex_bump} and the state running cost, and does not depend on the relative scaling of the state an input costs. Specifically, we will assume that the finite horizon problem optimized by the practical receding horizon process is of the form
 \begin{equation}\label{eq:bump_mpc}
     \inf_{\tilde{u}(\cdot)} \int_{0}^{T} q\|\tilde{x}\|_2^{2} + r\|\tilde{u}\|_2^2 dt + \|\tilde{x}_1(T)\|_2^2
 \end{equation}
 where $(\tilde{x}(\cdot), \tilde{u}(\cdot))$ solves \eqref{eq:ex_bump}, and will identify an equilibrium point which persists for each $r,T>0$.
 \twnote{We can show the following for this problem 1) that there exists an equilibrium point where $\PRHC$ gets stuff for every value of $q,r>0$ 2) the geometric reason for this is that the state running cost in non-convex in the linearizing coordinates}. 
 
 
 \begin{comment}
 To gain some informal intuition for where this equilibrium resides, consider the following problem:
\begin{align*}
    \inf_{\tilde{u}(\cdot)}&\int_{0}^{\infty} \|x \|_2^2 + r\|u \|_2^2 dt \\
    &\text{s.t. } \dot{x} = Ax + Bu + d 
\end{align*}
This can be thought of as the limit of \eqref{eq:bump_mpc} as $T \to \infty$ when trajectories of the system resided in $D_2$. Note that the value returned by this optimization is infinite since the origin is not an equilibrium point of $\dot{x} =Ax +Bu +d$. However, the cost 
\end{comment}


\subsection{1-D Driftless Systems}
\twnote{Will show that RHC converges for 1D driftless systems without the assumption that $g(x) =const$.}



==> proofs_two.tex <==
%!TEX root = LCSS_main_max.tex


\begin{proof}[\textbf{Proof of \Cref{lem:underbound}}] Under \Cref{ass:v_field_regularity,ass:eq_point}, we have that $\|\ddt \tilde{x}(t)\| = \|F(\tilde{x}(t),\tilde{u}(t))\| \le L_F(\|\tilde{x}(t)\| + \|\tilde{u}(t)\|)$. Hence, $|\ddt \|\tilde{x}(t)\|^2| = |\langle \tilde{x}(t), \ddt \tilde{x}(t) \rangle| \le L_F\|\tilde{x}(t)\|^2 + L_F \|\tilde{u}(t)\|\|\tilde{x}(t)\|$, which  at most $\frac{3L_F}{2}\|\tilde{x}(t)\|^2 + \frac{L_F}{2}\|\tilde{u}(t)\|^2$ by the AM-GM inequality. \Cref{asm:cost_smooth} then implies this is at most $\frac{c_1}{2\alpha_Q} (Q(\tilde{x}(t)) + R(\tilde{u}(t))$, where we define $c_1 := L_F(3+\frac{\alpha_Q }{ \alpha_R})$. Thus, given any times $s_1 \le s_2 \in [0,T]$, we have
\begin{align}
&\left|\|\tilde{x}(s_1)\|^2 - \|\tilde{x}(s_2)\|^2\right| \le  \int_{t=s_1}^{s_2} \left|\tfrac{\rmd}{\rmd t}\|\tilde{x}(t)\|^2\right| \rmd t \nonumber\\
&\quad  \le \tfrac{c_1}{2\alpha_Q}   \int_{t=s_1}^{s_2}(Q(\tilde{x}(t)) + R(\tilde{u}(t))\dt \le \tfrac{c_1}{2\alpha_Q} \Vtil(s_1) \label{eq:underbound_first_bound}.
\end{align}

To conclude, fix a time $s \in [0,T]$. We consider two cases: \textbf{Case 1:} There is a time $\tau \in [s,T]$ such that $\|\tilde{x}(\tau)\|^2 \le \frac{1}{2}\|\tilde{x}(s)\|^2$. Invoking \eqref{eq:underbound_first_bound},
\begin{align*}
&\tfrac{1}{2}\|\tilde{x}(s)\|^2 \ge  \left|\|\tilde{x}(s)\|^2 -  \|\tilde{x}(\tau)\|^2\right| \\
&\quad \ge  \left|\|\tilde{x}(s)\|^2 - \|\tilde{x}(s\tau)\|^2\right| \ge \tfrac{c_1}{2\alpha_Q} \Vtil(s).
\end{align*}
\textbf{Case 2:} There is no such time $\tau$, so $\|\tilde{x}(t)\|^2 \ge \frac{1}{2}\|\tilde{x}(s)\|^2$ for all $t \in [s,T]$. In this case, $\Vtil(s) \ge \alpha_Q \int_{t=s}^T \|\tilde{x}(t)\|^2 \rmd t + \alpha_V\|\tilde{x}(T)^2\| \ge (\alpha_Q(T-s) + \alpha_V)\cdot\|\tilde{x}(s)\|^2/2$. Inverting, and combining both cases,
\begin{align}
\|\tilde{x}(s)\|^2 \le \frac{1}{\alpha_Q}\max\{c_1, \tfrac{2}{T-s + \alpha_V/\alpha_Q}\}\Vtil(s)  \label{eq:intermediate}
\end{align} 
Finally, for any $s' \in [0,s]$, arguing as in \eqref{eq:underbound_first_bound}, and applying \eqref{eq:intermediate} and some simplifications (incuding $\Vtil(s') \ge \Vtil(s)$),
\begin{align*}
\|\xtil(s)\|^2 &\le \|\xtil(s')\|^2 + |\int_{t=s'}^{s} (\tfrac{\rmd}{\rmd t}\|\tilde{x}(t)\|^2) \rmd t|\\
&\le \|\xtil(s')\|^2 + \frac{c_1}{2\alpha_Q}\Vtil(s')\\
&\le \frac{1}{\alpha_Q}\underbrace{(2c_1 + 2\tfrac{1}{T-(s') + \frac{\alpha_V}{\alpha_Q}})}_{:=\calC_0(s')}\Vtil(s').
\end{align*}
\end{proof}


In view of \Cref{lem:comparison}, to obtain a bound on $\Vtil(s)$ it suffices to bound  $\Vjacst(s) :=\inf_{\ubar_{[s,T]}} \Jlin_{T-s}(\cdot, ~ \xtil(s), \util_{[s,T]})$. Moreover, we can bound $\Vjacst(s)$ by bounding $\Jlin_{T-s}(\ubar_{[s,T]};~ \xtil(t), \util_{[s,T]})$ for any (possibly suboptimal) control $\ubar_{[s,T]}$; for simplicity, let us drop the ${[s,T]}$-subscript going forward. We select $\ubar(t) = \ubar_1(t) + \ubar_2(t)$, where $\ubar_1(t)$ satisfies $\Btil(t) \ubar_1(t) =- \tilde{d}(t)$, and where $\ubar_2$ witnesses $\gamma$-stabilizability at time $s$ as in \Cref{asm:stabilizable}.

With this choice of $\ubar(t)$ the dynamics of $\xbar(t)$ in $\Jlin_{T-s}$  are $\tfrac{\rmd}{\rmd t} \xbar(t) = \Atil(t)\xbar(t) + \Btil(t)\ubar(t) + \tilde{d}(t) = \Atil(t)\xbar(t) + \Btil \bar{u}_2(t)$, and, writing out $\Jlin_{T-s}$ explicitly, we obtain
\begin{align} 
\Vjacst(s) \le \textstyle \int_{t=s}^T (Q(\xbar(t)) + R(\ubar(t))\rmd t + V(\xbar(T)).
\end{align}
By the elementary bound $\|\ubar(t)\|^2 \le 2\|\ubar_1(t)\|^2 + 2\|\bar{u}_2(t)\|^2$, the following holds for constant $c = \max\{\beta_V,2\beta_R,\beta_Q\}$,
\begin{align}\textstyle
&\Vjacst(s)\textstyle\le   2\beta_R \int_{t=s}^T \|\ubar_1(t)\|^2 \dt \label{eq:P_line_one}\\
&\quad+c \left(\textstyle\int_{t=s}^T (\|\xbar(t)\|^2 + \|\ubar(t)\|^2)\rmd t + \|\xbar(T)\|^2\right). \label{eq:P_line_two}
\end{align}
To bound \eqref{eq:P_line_two}, we observe that $\ddt \xbar(t) = \Atil(t)\xbar(t) + \Btil(t)\ubar(t) + \tilde{d}(t) = \Atil(t)\xbar(t) + \Btil(t)\bar{u}_2(t)$, which corresponds to the $\hat{x}(t)$ dynamics in the definion of $\gamma$-stabilizability; thus, \eqref{eq:P_line_two} is at most $c \cdot \gamma \|\xtil(s)\|^2$. 

To bound \eqref{eq:P_line_one}, we use \eqref{asm:linearizable_bound} to bound $ \|\ubar_1(t)\|^2 \le  2L_x^2\|\xtil(t)\|^2 + 2 L_u^2\|\util(t)\|^2 \le 2c'(Q(\xtil(t)) +  R(\util(t))/\beta_R$, where $c' =  \beta_R\max\{\frac{L_x^2}{\alpha_Q},\frac{ L_u^2}{\alpha_R})$. Hence,  in view of \Cref{lem:comparison}, and the principle of optimality:
\begin{align*}
& 2 \beta_R\textstyle\int_{t=s}^T \|\bar{u}_1(t)\|^2 \dt \le  4c'\beta_R \textstyle\int_{t=s}^T (Q(\xtil(t)) +  R(\util(t))\dt \\
&\quad \le  4c' \beta_R \Vtil(s)  \le 4c'\beta_R(\Vjacst(s)  + \tfrac{\epsilon^2}{2\alpha_R})
\end{align*}
Putting the bounds together and rearranging:
\begin{align*}
(1-   4 \beta_R c' )\Vjacst(s) \le c \cdot \gamma \|\xtil(s)\|^2 + \tfrac{2 c'\beta_R}{ \alpha_R} \epsilon^2
\end{align*}
Under \Cref{asm:linearizable_compatibility}, we have $4\beta_R c'\le 1/2$, so that
\begin{align}
\Vjacst(s) \le 2c\cdot \gamma \|\xtil(s)\|^2 + \tfrac{4 c'\beta_R}{\alpha_R} \epsilon^2.
\end{align}
We recognize $2c\gamma \le \calC_1$, and $\tfrac{4 c' \beta_R}{\alpha_R} = \calC_2 - \frac{1}{2\alpha_R}$, and invoke \Cref{lem:comparison} to obtain the desired bound. \qedd


\begin{proof}[\textbf{Proof of \Cref{thm:RHC}}]
We first assume that $\alpha_V>0$ and bound the rate of covegence in terms of $\calC_0$; the steps of the proof can be repeated by replacing $\calC_0$ with $\calC_0^\delta$ throughout and then applying the tighter of the two bounds. 

For each $k \in \N$ we will let $\tilde{J}_{k} = J_T(\tilde{u}_{k}(\cdot;x_0,\uwarm_0),x_0)$ and $\tilde{J}_{k} = J_T(\tilde{u}_{k}(\cdot;x_0,\uwarm_0),x_0)$. Respectively, these are the cost incurred by the $k$-th planning solution and the $k$-th warm-start initial guess. For simplicity, we drop the dependence on $x_0$ and $\bar{u}_0$ from here on. We also let $(\tilde{x}_k(\cdot),\tilde{u}(\cdot))$ and $(\bar{x}_k(\cdot),\bar{u}_k(\cdot))$ denote the corresponding system trajectories. 
Our goal is to show that the sequence of losses $\set{\tilde{J}_k}_{k=1}^{\infty}$ is geometrically decreasing. Indeed, using property $1)$ of \Cref{asm:planner} we have

\begin{align}\label{eq:tot_bound}
\tilde{J}_{T}^{k+1} &\leq \bar{J}_{T}^{k+1} = \bar{J}_{T}^{k+1} - \tilde{J}_T^{k} + \tilde{J}_T^k\\\nonumber
&=\int_{T-\delta}^{T}Q(\bar{x}_{k+1}(\tau)) +R(\bar{u}_{k+1}(\tau))d\tau + V(\bar{x}_{k+1}(T))\\ \nonumber
&-\int_{0}^\delta Q(\tilde{x}_k(\tau)) +R(\tilde{u}_k(\tau))d \tau - V(\tilde{x}_k(T)) + \tilde{J}_{T}^k\\ \nonumber
&\leq \int_{T-\delta}^{T}\alpha_{Q}\|\bar{x}_{k+1}(\tau)\|_2^2  + \alpha_{V}\|\bar{x}_{k+1}(T))\|_2^2 \\ \nonumber
&+  \left( e^{-\frac{\delta}{\calC_1}} + \frac{\alpha_Q}{2}\calC_2  \epsilon_0^2\right)\tilde{J}_k
\end{align}
where the second inequality follows from \Cref{asm:cost_smooth}, the fact that $\bar{u}_{k+1}(t) = 0$ for each $t \in \sp{T-\delta, T}$, and applying the second inequality in \eqref{eq:exp_value_bound} which shows that $J_{T-\delta}(\tilde{u}_k|_{\sp{\delta,T}}, \tilde{x}_k(\delta)) \leq e^{-\frac{\delta}{\calC_1}}\tilde{J}_k + \frac{\alpha_Q}{2} \calC_2 \epsilon_0^2 \tilde{J}_k)$, where we have also used property $2)$ of \Cref{asm:planner}. The second fact also implies that $|\dot{\bar{x}}_{k+1}(t) = |F(x_{k+1}(t), 0)| \leq L_F|\bar{x}(\bar{x}(t))|$ (by \Cref{ass:v_field_regularity}) for each $t\in \sp{T-\delta, T}$. Thus, by a standard application of a Gronwall-type inequality for each $t \in \sp{T-\delta, T}$ we have will will have 
\begin{align}\label{eq:term_bound}
\|\bar{x}_{k+1}(t)\|_2^2 &\leq e^{2L_F \delta} \|\bar{x}_{k+1}(T-\delta)\|_2^2\\
&\leq e^{2L_F\delta} \calC_0\left(\calC_1e^{-\frac{T-\delta}{\calC_1}}\tilde{J}_k + \frac{1}{2}\calC_2\epsilon_0^
2 \tilde{J}_k\right)
\end{align}
where we have used the fact that $\tilde{x}_{k}(T-\delta) = \bar{x}_{k+1}(T-\delta)$, property $2$ from \Cref{asm:planner} and \Cref{thm:plan}. Combining the above observations with the final inequality in \eqref{eq:tot_bound},integrating, and rearranging terms, and simplifying provides
\begin{multline}
\tilde{J}_{k+1} \leq \bigg(e^{-\frac{\delta}{\calC_1}} + \calC_0\bigg[\calC_1e^{2L_F\delta}(\delta \alpha_{Q} + \alpha_V)e^{-\frac{T-\delta}{\calC_1}}    \\ + \frac{1}{2}e^{2L_F\delta}((\delta +1)\alpha_Q + \alpha_V) \calC_2  \epsilon_0^2 \bigg]\bigg)\tilde{J}_k
\end{multline}
Which simplifies to 
\begin{equation}\label{eq:geometric_decay}
\tilde{J}_{k+1} \leq \left(e^{-\frac{\delta}{\calC_1}} + \left[\mathcal{T}(\delta,T) + \mathcal{E}(\delta, \epsilon_0)\right]\right)\tilde{J}_{k}.
\end{equation}
 This geometric decay implies that 
\begin{equation}
J_T(\tilde{u}_k(0), \tilde{x}_k(0)) \leq  e^{ 2\eta(\delta, T,\epsilon_0) t_k} J_T(\tilde{u}_0(0), \tilde{x}_0(0))
\end{equation}
This can then be converted into the desired bound on the state trajectory by applying \Cref{lem:underbound,lem:overbound}.
\end{proof}

